Sensing-Throughput Tradeoff for Interweave Cognitive Radio System: A Deployment-Centric Viewpoint

Secondary access to the licensed spectrum is viable only if interference is avoided at the primary system. In this regard, different paradigms have been conceptualized in the existing literature. Of these, Interweave Systems (ISs) that employ spectrum sensing have been widely investigated. Baseline models investigated in the literature characterize the performance of IS in terms of a sensing-throughput tradeoff, however, this characterization assumes the knowledge of the involved channels at the secondary transmitter, which is unavailable in practice. Motivated by this fact, we establish a novel approach that incorporates channel estimation in the system model, and consequently investigate the impact of imperfect channel estimation on the performance of the IS. More particularly, the variation induced in the detection probability affects the detector's performance at the secondary transmitter, which may result in severe interference at the primary users. In this view, we propose to employ average and outage constraints on the detection probability, in order to capture the performance of the IS. Our analysis reveals that with an appropriate choice of the estimation time determined by the proposed model, the degradation in performance of the IS can be effectively controlled, and subsequently the achievable secondary throughput can be significantly enhanced.

==> Makefile <==
ps_2C: paper_2C.tex refs.bib
	latex paper_2C.tex
	bibtex paper_2C
	latex paper_2C.tex
	dvips paper_2C.dvi -o paper_2C.ps
	ps2pdf paper_2C.ps

pdf_2C: paper_2C.tex refs.bib
	pdflatex paper_2C.tex
	bibtex paper_2C
	pdflatex paper_2C.tex

# Only for embedding pdf fonts
pdf_EF_2C: paper_2C.tex refs.bib 
	pdflatex paper_2C.tex
	bibtex paper_2C
	pdflatex paper_2C.tex
	# convert to Postscript
	pdftops paper_2C.pdf paper_2C.ps
	# reconvert to PDF but enforce font embedding (note, hyperlinks will not survive)
	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true paper_2C.ps paper_2C.pdf
	# verify
	pdffonts paper_2C.pdf

clean_2C:
	rm *.log *.aux *.bbl *.blg paper_2C.pdf *.ps *.dvi *.out

cp_complete_2C:
	cp -rf ../Ext_CrownCom2015/ ~/Dropbox 	


cp_paper_2C:
	cp -rf paper_2C.tex paper_2C.pdf refs.bib figures/ SourceFiles ~/Dropbox/Ext_CrownCom2015/ 	



cp_resp:
	cp -rf ./response\ letter/* ~/Dropbox/Ext_CrownCom2015/response\ letter/	


==> figures/fig_C_0_approx_vs_rho_s_diff_SNR.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_C_0_approx_vs_rho_s_diff_SNR}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           02-Apr-2015 08:47:49
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\fontsize{11}{16.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\C0$\end{tabular}}%
\psfrag{s06}[t][t]{\fontsize{11}{16.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rho_s$ = [ms]\end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Simulated}%
\psfrag{s13}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Theoretical}%
\psfrag{s14}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Simulated}%
%
% axes font properties:
\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.1}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.3}%
\psfrag{x04}[t][t]{0.4}%
\psfrag{x05}[t][t]{0.5}%
\psfrag{x06}[t][t]{0.6}%
\psfrag{x07}[t][t]{0.7}%
\psfrag{x08}[t][t]{0.8}%
\psfrag{x09}[t][t]{0.9}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
\psfrag{v06}[r][r]{2.5}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_C_0_approx_vs_rho_s_diff_SNR.eps}}%
%\end{psfrags}%
%
% End fig_C_0_approx_vs_rho_s_diff_SNR.tex


==> figures/fig_C_1_approx_vs_rho_p_diff_SNR.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_C_1_approx_vs_rho_p_diff_SNR}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           05-Jul-2015 15:48:10
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\fontsize{11}{16.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\Co$\end{tabular}}%
\psfrag{s06}[t][t]{\fontsize{11}{16.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rho_p$ = [ms]\end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Simulated}%
\psfrag{s13}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Theoretical}%
\psfrag{s14}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Simulated}%
%
% axes font properties:
\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.1}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.3}%
\psfrag{x04}[t][t]{0.4}%
\psfrag{x05}[t][t]{0.5}%
\psfrag{x06}[t][t]{0.6}%
\psfrag{x07}[t][t]{0.7}%
\psfrag{x08}[t][t]{0.8}%
\psfrag{x09}[t][t]{0.9}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_C_1_approx_vs_rho_p_diff_SNR.eps}}%
%\end{psfrags}%
%
% End fig_C_1_approx_vs_rho_p_diff_SNR.tex


==> figures/fig_C_1_approx_vs_rho_s_diff_SNR.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_C_1_approx_vs_rho_s_diff_SNR}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           02-Apr-2015 08:45:51
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\fontsize{11}{16.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\C1$\end{tabular}}%
\psfrag{s06}[t][t]{\fontsize{11}{16.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rho_s$ = [ms]\end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Simulated}%
\psfrag{s13}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Theoretical}%
\psfrag{s14}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Simulated}%
%
% axes font properties:
\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.1}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.3}%
\psfrag{x04}[t][t]{0.4}%
\psfrag{x05}[t][t]{0.5}%
\psfrag{x06}[t][t]{0.6}%
\psfrag{x07}[t][t]{0.7}%
\psfrag{x08}[t][t]{0.8}%
\psfrag{x09}[t][t]{0.9}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_C_1_approx_vs_rho_s_diff_SNR.eps}}%
%\end{psfrags}%
%
% End fig_C_1_approx_vs_rho_s_diff_SNR.tex


==> figures/fig_opt_P_d_vs_SNR_AWGN.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_opt_P_d_vs_SNR_AWGN}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           29-Oct-2015 06:37:13
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\pd$\end{tabular}}%
\psfrag{s06}[t][t]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\snrrcvd$ [dB]\end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trsoc$}%
\psfrag{s13}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trs$}%
\psfrag{s14}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trsac$}%
\psfrag{s15}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trsoc$}%
%
% axes font properties:
\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-15}%
\psfrag{x02}[t][t]{-10}%
\psfrag{x03}[t][t]{-5}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{5}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.978}%
\psfrag{v02}[r][r]{0.98}%
\psfrag{v03}[r][r]{0.982}%
\psfrag{v04}[r][r]{0.984}%
\psfrag{v05}[r][r]{0.986}%
\psfrag{v06}[r][r]{0.988}%
\psfrag{v07}[r][r]{0.99}%
\psfrag{v08}[r][r]{0.992}%
\psfrag{v09}[r][r]{0.994}%
\psfrag{v10}[r][r]{0.996}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_opt_P_d_vs_SNR_AWGN.eps}}%
%\end{psfrags}%
%
% End fig_opt_P_d_vs_SNR_AWGN.tex


==> figures/fig_opt_P_f_vs_SNR_AWGN.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_opt_P_f_vs_SNR_AWGN}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           20-Jul-2015 16:49:26
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\pd$\end{tabular}}%
\psfrag{s06}[t][t]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\snrrcvd$ [dB]\end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trsoc$}%
\psfrag{s13}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trs$}%
\psfrag{s14}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trsac$}%
\psfrag{s15}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trsoc$}%
%
% axes font properties:
\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-15}%
\psfrag{x02}[t][t]{-10}%
\psfrag{x03}[t][t]{-5}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{5}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.1}%
\psfrag{v02}[r][r]{0.2}%
\psfrag{v03}[r][r]{0.3}%
\psfrag{v04}[r][r]{0.4}%
\psfrag{v05}[r][r]{0.5}%
\psfrag{v06}[r][r]{0.6}%
\psfrag{v07}[r][r]{0.7}%
\psfrag{v08}[r][r]{0.8}%
\psfrag{v09}[r][r]{0.9}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_opt_P_f_vs_SNR_AWGN.eps}}%
%\end{psfrags}%
%
% End fig_opt_P_f_vs_SNR_AWGN.tex


==> figures/fig_opt_thr_vs_est_time_AWGN.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_opt_thr_vs_est_time_AWGN}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           04-Jul-2015 08:28:36
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\trs$ [bits/sec/Hz]\end{tabular}}%
\psfrag{s06}[t][t]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\test$ [ms]\end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Opt. $\ttest$}%
\psfrag{s13}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trs$}%
\psfrag{s14}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trsac$}%
\psfrag{s15}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\trsoc$}%
\psfrag{s16}[l][l]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Opt. $\ttest$}%
%
% axes font properties:
\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{3}%
\psfrag{x04}[t][t]{4}%
\psfrag{x05}[t][t]{5}%
\psfrag{x06}[t][t]{6}%
\psfrag{x07}[t][t]{7}%
\psfrag{x08}[t][t]{8}%
\psfrag{x09}[t][t]{9}%
\psfrag{x10}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{1.5}%
\psfrag{v04}[r][r]{2}%
\psfrag{v05}[r][r]{2.5}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_opt_thr_vs_est_time_AWGN.eps}}%
%\end{psfrags}%
%
% End fig_opt_thr_vs_est_time_AWGN.tex

